3D Point Cloud Registration with Learning-based Matching Algorithm

We present a novel differential matching algorithm for 3D point cloud registration. Instead of only optimizing the feature extractor for a matching algorithm, we propose a learning-based matching module optimized to the jointly-trained feature extractor. We focused on edge-wise feature-forwarding architectures, which are memory-consuming but can avoid the over-smoothing effect that GNNs suffer. We improve its memory efficiency to scale it for point cloud registration while investigating the best way of connecting it to the feature extractor. Experimental results show our matching module's significant impact on performance improvement in rigid/non-rigid and whole/partial point cloud registration datasets with multiple contemporary feature extractors. For example, our module boosted the current SOTA method, RoITr, by +5.4%, and +7.2% in the NFMR metric and +6.1% and +8.5% in the IR metric on the 4DMatch and 4DLoMatch datasets, respectively.

==> Text/Limitation.tex <==
\section{Limitation}
The first remarkable limitation of our approach is the sensitivity to the hyperparameter $r$. As with the other point cloud processing methods~\cite{ravanbakhsh2016deep,liu2020semantic,jiang2020end}, our ESFW module is also subject to negative effects in a particular hyperparameter setting. Specifically, as shown in tables~\ref{Table.4DMatch_r},~\ref{Table.4DLoMatch_r},~\ref{Table.3DMatch_r}, and~\ref{Table.3DLoMatch_r}, it is crucial to select a suitable value of $r$, which is the threshold value of edge selection. Too small $r$ can eliminate the edge toward the corresponding node, whereas too large $r$ can lead to leave valueless edges, which made unnecessary memory consumption and performance degradation. To overcome this limitation, further architectural improvements are needed. \par
The second limitation is memory usage as shown in point cloud processing~\cite{wang2018sgpn,liu2019dynamic} and graph neural networks~\cite{wu2020comprehensive,klicpera2018predict}. Our ESFW module process graphs with edge information, and its memory usage thus becomes larger in proportion with the numbers of input points $N$ and the threshold value of edge selection $r$. Because this limitation is closely related to the first limitation, it is important to consider an ideal architecture in terms of both limitations. Note that, since the selection of $r$ is conducted based on the extracted features, we believe that the architecture should be considered not only for our ESFW module but also for the point cloud feature extractor.%%
